Benchmarking Large Language Models for Math Reasoning Tasks

The use of Large Language Models (LLMs) in mathematical reasoning has become a cornerstone of related research, demonstrating the intelligence of these models and enabling potential practical applications through their advanced performance, such as in educational settings. Despite the variety of datasets and in-context learning algorithms designed to improve the ability of LLMs to automate mathematical problem solving, the lack of comprehensive benchmarking across different datasets makes it complicated to select an appropriate model for specific tasks. In this project, we present a benchmark that fairly compares seven state-of-the-art in-context learning algorithms for mathematical problem solving across five widely used mathematical datasets on four powerful foundation models. Furthermore, we explore the trade-off between efficiency and performance, highlighting the practical applications of LLMs for mathematical reasoning. Our results indicate that larger foundation models like GPT-4o and LLaMA 3-70B can solve mathematical reasoning independently from the concrete prompting strategy, while for smaller models the in-context learning approach significantly influences the performance. Moreover, the optimal prompt depends on the chosen foundation model. We open-source our benchmark code to support the integration of additional models in future research.

==> taxonomy/taxonomy.tex <==


% % \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
% % %uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

% % %Rounded Rect "Main"
% % \draw   (30.1,205.83) .. controls (27.01,205.83) and (24.5,203.33) .. (24.5,200.23) -- (24.5,54.27) .. controls (24.5,51.17) and (27.01,48.67) .. (30.1,48.67) -- (46.9,48.67) .. controls (49.99,48.67) and (52.5,51.17) .. (52.5,54.27) -- (52.5,200.23) .. controls (52.5,203.33) and (49.99,205.83) .. (46.9,205.83) -- cycle ;

% % %Rounded Rect "Strategy"
% % \draw   (98.2,53.36) .. controls (98.2,50.8) and (100.27,48.73) .. (102.83,48.73) -- (284.04,48.73) .. controls (286.6,48.73) and (288.67,50.8) .. (288.67,53.36) -- (288.67,67.24) .. controls (288.67,69.8) and (286.6,71.87) .. (284.04,71.87) -- (102.83,71.87) .. controls (100.27,71.87) and (98.2,69.8) .. (98.2,67.24) -- cycle ;

% % %Rounded Rect [id:dp13334423244616878] 
% % \draw   (97.47,165.87) .. controls (97.47,163.29) and (99.56,161.2) .. (102.13,161.2) -- (282,161.2) .. controls (284.58,161.2) and (286.67,163.29) .. (286.67,165.87) -- (286.67,179.87) .. controls (286.67,182.44) and (284.58,184.53) .. (282,184.53) -- (102.13,184.53) .. controls (99.56,184.53) and (97.47,182.44) .. (97.47,179.87) -- cycle ;

% % %Rounded Rect [id:dp06746547135445946] 
% % \draw   (337.33,21.03) .. controls (337.33,18.32) and (339.52,16.13) .. (342.23,16.13) -- (522.04,16.13) .. controls (524.74,16.13) and (526.93,18.32) .. (526.93,21.03) -- (526.93,35.71) .. controls (526.93,38.41) and (524.74,40.6) .. (522.04,40.6) -- (342.23,40.6) .. controls (339.52,40.6) and (337.33,38.41) .. (337.33,35.71) -- cycle ;

% % %Rounded Rect [id:dp5597732074812531] 
% % \draw   (336.6,52.41) .. controls (336.6,49.76) and (338.76,47.6) .. (341.41,47.6) -- (522.99,47.6) .. controls (525.64,47.6) and (527.8,49.76) .. (527.8,52.41) -- (527.8,66.85) .. controls (527.8,69.51) and (525.64,71.67) .. (522.99,71.67) -- (341.41,71.67) .. controls (338.76,71.67) and (336.6,69.51) .. (336.6,66.85) -- cycle ;

% % %Rounded Rect [id:dp16394219746751593] 
% % \draw   (336.8,83) .. controls (336.8,80.39) and (338.92,78.27) .. (341.53,78.27) -- (522.73,78.27) .. controls (525.35,78.27) and (527.47,80.39) .. (527.47,83) -- (527.47,97.2) .. controls (527.47,99.81) and (525.35,101.93) .. (522.73,101.93) -- (341.53,101.93) .. controls (338.92,101.93) and (336.8,99.81) .. (336.8,97.2) -- cycle ;

% % %Rounded Rect [id:dp5718262152901658] 
% % \draw   (335.13,134.11) .. controls (335.13,131.47) and (337.27,129.33) .. (339.91,129.33) -- (520.96,129.33) .. controls (523.6,129.33) and (525.73,131.47) .. (525.73,134.11) -- (525.73,148.43) .. controls (525.73,151.06) and (523.6,153.2) .. (520.96,153.2) -- (339.91,153.2) .. controls (337.27,153.2) and (335.13,151.06) .. (335.13,148.43) -- cycle ;

% % %Rounded Rect [id:dp9434376311423853] 
% % \draw   (334.47,165.49) .. controls (334.47,162.9) and (336.57,160.8) .. (339.16,160.8) -- (520.77,160.8) .. controls (523.37,160.8) and (525.47,162.9) .. (525.47,165.49) -- (525.47,179.57) .. controls (525.47,182.17) and (523.37,184.27) .. (520.77,184.27) -- (339.16,184.27) .. controls (336.57,184.27) and (334.47,182.17) .. (334.47,179.57) -- cycle ;

% % %Rounded Rect [id:dp4670795319787643] 
% % \draw   (334.73,196.69) .. controls (334.73,194.1) and (336.83,192) .. (339.43,192) -- (520.04,192) .. controls (522.63,192) and (524.73,194.1) .. (524.73,196.69) -- (524.73,210.77) .. controls (524.73,213.37) and (522.63,215.47) .. (520.04,215.47) -- (339.43,215.47) .. controls (336.83,215.47) and (334.73,213.37) .. (334.73,210.77) -- cycle ;

% % %Straight Lines [id:da8342548459829764] 
% % \draw    (52,115.56) -- (68.67,115.56) ;
% % %Straight Lines [id:da264346558430124] 
% % \draw    (70,174.22) -- (70,58.89) ;
% % %Straight Lines [id:da3482901118358255] 
% % \draw    (70,58.89) -- (98,58.89) ;
% % %Straight Lines [id:da8185169417510957] 
% % \draw    (70,174.22) -- (98,174.22) ;
% % %Straight Lines [id:da5970599654535012] 
% % \draw    (307.33,89.22) -- (307.67,27.89) ;
% % %Straight Lines [id:da5677947405832151] 
% % \draw    (307.67,27.89) -- (335.67,27.89) ;
% % %Straight Lines [id:da08109115639970066] 
% % \draw    (307.33,89.22) -- (335.33,89.22) ;
% % %Straight Lines [id:da603888173433695] 
% % \draw    (288,58.22) -- (335.5,58.56) ;
% % %Straight Lines [id:da9668122023481845] 
% % \draw    (306,202.56) -- (306.33,141.22) ;
% % %Straight Lines [id:da41181555222193966] 
% % \draw    (306.33,141.22) -- (334.33,141.22) ;
% % %Straight Lines [id:da1746421482121866] 
% % \draw    (306,202.56) -- (334,202.56) ;
% % %Straight Lines [id:da5073022594694027] 
% % \draw    (286.67,171.56) -- (334.17,171.89) ;
% % %Rounded Rect [id:dp08565300826534117] 
% % \draw   (557.33,21.89) .. controls (557.33,19.19) and (559.52,17) .. (562.23,17) -- (921.77,17) .. controls (924.48,17) and (926.67,19.19) .. (926.67,21.89) -- (926.67,36.57) .. controls (926.67,39.28) and (924.48,41.47) .. (921.77,41.47) -- (562.23,41.47) .. controls (559.52,41.47) and (557.33,39.28) .. (557.33,36.57) -- cycle ;

% % %Rounded Rect [id:dp36019398419840787] 
% % \draw   (557,54.89) .. controls (557,52.19) and (559.19,50) .. (561.89,50) -- (921.44,50) .. controls (924.14,50) and (926.33,52.19) .. (926.33,54.89) -- (926.33,69.57) .. controls (926.33,72.28) and (924.14,74.47) .. (921.44,74.47) -- (561.89,74.47) .. controls (559.19,74.47) and (557,72.28) .. (557,69.57) -- cycle ;
% % %Rounded Rect [id:dp990284470711138] 
% % \draw   (557.33,85.89) .. controls (557.33,83.19) and (559.52,81) .. (562.23,81) -- (921.77,81) .. controls (924.48,81) and (926.67,83.19) .. (926.67,85.89) -- (926.67,100.57) .. controls (926.67,103.28) and (924.48,105.47) .. (921.77,105.47) -- (562.23,105.47) .. controls (559.52,105.47) and (557.33,103.28) .. (557.33,100.57) -- cycle ;
% % %Rounded Rect [id:dp7385353967632635] 
% % \draw   (555,136.89) .. controls (555,134.19) and (557.19,132) .. (559.89,132) -- (919.44,132) .. controls (922.14,132) and (924.33,134.19) .. (924.33,136.89) -- (924.33,151.57) .. controls (924.33,154.28) and (922.14,156.47) .. (919.44,156.47) -- (559.89,156.47) .. controls (557.19,156.47) and (555,154.28) .. (555,151.57) -- cycle ;
% % %Rounded Rect [id:dp09911027124281035] 
% % \draw   (556,167.89) .. controls (556,165.19) and (558.19,163) .. (560.89,163) -- (920.44,163) .. controls (923.14,163) and (925.33,165.19) .. (925.33,167.89) -- (925.33,182.57) .. controls (925.33,185.28) and (923.14,187.47) .. (920.44,187.47) -- (560.89,187.47) .. controls (558.19,187.47) and (556,185.28) .. (556,182.57) -- cycle ;
% % %Rounded Rect [id:dp9760277717365602] 
% % \draw   (555,197.89) .. controls (555,195.19) and (557.19,193) .. (559.89,193) -- (919.44,193) .. controls (922.14,193) and (924.33,195.19) .. (924.33,197.89) -- (924.33,212.57) .. controls (924.33,215.28) and (922.14,217.47) .. (919.44,217.47) -- (559.89,217.47) .. controls (557.19,217.47) and (555,215.28) .. (555,212.57) -- cycle ;
% % %Straight Lines [id:da8107566291187137] 
% % \draw    (527.67,27.89) -- (555.67,27.89) ;
% % %Straight Lines [id:da5019077435241249] 
% % \draw    (529.67,59.89) -- (557.67,59.89) ;
% % %Straight Lines [id:da15043617991990343] 
% % \draw    (529.33,89.89) -- (557.33,89.89) ;
% % %Straight Lines [id:da8401352624791865] 
% % \draw    (527.67,142.89) -- (555.67,142.89) ;
% % %Straight Lines [id:da41225016458038355] 
% % \draw    (525.47,174.57) -- (553.47,174.57) ;
% % %Straight Lines [id:da3829448090452344] 
% % \draw    (528,203.89) -- (556,203.89) ;

% % % Text Node
% % \draw (344.4,81.27) node [anchor=north west][inner sep=0.75pt]   [align=left] {External Engine};
% % % Text Node
% % \draw (344.2,50.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Process Optimization};
% % % Text Node
% % \draw (342.73,132.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {Task-specific Fine-Tuning};
% % % Text Node
% % \draw (105.07,51.73) node [anchor=north west][inner sep=0.75pt]   [align=left] {Strategy Enhanced};
% % % Text Node
% % \draw (105.07,164.2) node [anchor=north west][inner sep=0.75pt]   [align=left] {Knowledge Enhanced};
% % % Text Node
% % \draw (342.33,195) node [anchor=north west][inner sep=0.75pt]   [align=left] {Imitation Learning};
% % % Text Node
% % \draw (344.93,19.13) node [anchor=north west][inner sep=0.75pt]   [align=left] {Prompt Engineering};
% % % Text Node
% % \draw (342.07,163.8) node [anchor=north west][inner sep=0.75pt]   [align=left] {Further Pre-Training};
% % % Text Node
% % \draw (29.5,198.23) node [anchor=north west][inner sep=0.75pt]  [rotate=-270] [align=left] {{\small Math Reasoning with LLMs}};
% % % Text Node
% % \draw (563.93,55) node [anchor=north west][inner sep=0.75pt]   [align=left] {SelfConsistency-CoT [], Complex-CoT []};
% % % Text Node
% % \draw (564.23,20) node [anchor=north west][inner sep=0.75pt]   [align=left] {CoT [], ZeroShot-CoT [], Auto-CoT [], Least-to-most []};
% % % Text Node
% % \draw (564.23,84) node [anchor=north west][inner sep=0.75pt]   [align=left] {PAL [], PoT []};
% % % Text Node
% % \draw (561.89,135) node [anchor=north west][inner sep=0.75pt]   [align=left] {LLema [], MAmmoTH [], MathCoder []};
% % % Text Node
% % \draw (562.89,166) node [anchor=north west][inner sep=0.75pt]   [align=left] {Lila []};
% % % Text Node
% % \draw (561.89,196) node [anchor=north west][inner sep=0.75pt]   [align=left] {ToRa []};


% % \end{tikzpicture}


% \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

% \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
% %uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300


% % %Rounded Rect "Main"
% %\draw   (30.1,205.83) .. controls (27.01,205.83) and (24.5,203.33) .. (24.5,200.23) -- (24.5,54.27) .. controls (24.5,51.17) and (27.01,48.67) .. (30.1,48.67) -- (46.9,48.67) .. controls (49.99,48.67) and (52.5,51.17) .. (52.5,54.27) -- (52.5,200.23) .. controls (52.5,203.33) and (49.99,205.83) .. (46.9,205.83) -- cycle ;

% %Rounded Rect [id:dp05318112641491435] 
% \draw   (35.43,203.83) .. controls (32.34,203.83) and (29.83,201.33) .. (29.83,198.23) -- (29.83,32.27) .. controls (29.83,29.17) and (32.34,26.67) .. (35.43,26.67) -- (52.23,26.67) .. controls (55.33,26.67) and (57.83,29.17) .. (57.83,32.27) -- (57.83,198.23) .. controls (57.83,201.33) and (55.33,203.83) .. (52.23,203.83) -- cycle ;

% %Rounded Rect [id:dp30580903458237174] 
% \draw   (84.87,54.03) .. controls (84.87,51.47) and (86.94,49.4) .. (89.49,49.4) -- (242.43,49.4) .. controls (244.98,49.4) and (247.06,51.47) .. (247.06,54.03) -- (247.06,67.91) .. controls (247.06,70.46) and (244.98,72.53) .. (242.43,72.53) -- (89.49,72.53) .. controls (86.94,72.53) and (84.87,70.46) .. (84.87,67.91) -- cycle ;

% %Rounded Rect [id:dp05443013590966794] 
% \draw   (84.13,166.53) .. controls (84.13,163.96) and (86.22,161.87) .. (88.8,161.87) -- (242.39,161.87) .. controls (244.97,161.87) and (247.06,163.96) .. (247.06,166.53) -- (247.06,180.53) .. controls (247.06,183.11) and (244.97,185.2) .. (242.39,185.2) -- (88.8,185.2) .. controls (86.22,185.2) and (84.13,183.11) .. (84.13,180.53) -- cycle ;
% %Rounded Rect [id:dp012347841356451505] 
% \draw   (269.67,24.03) .. controls (269.67,21.32) and (271.86,19.13) .. (274.56,19.13) -- (445.61,19.13) .. controls (448.31,19.13) and (450.5,21.32) .. (450.5,24.03) -- (450.5,38.71) .. controls (450.5,41.41) and (448.31,43.6) .. (445.61,43.6) -- (274.56,43.6) .. controls (271.86,43.6) and (269.67,41.41) .. (269.67,38.71) -- cycle ;
% %Rounded Rect [id:dp45468087205710206] 
% \draw   (269.6,55.41) .. controls (269.6,52.76) and (271.76,50.6) .. (274.41,50.6) -- (445.46,50.6) .. controls (448.12,50.6) and (450.28,52.76) .. (450.28,55.41) -- (450.28,69.85) .. controls (450.28,72.51) and (448.12,74.67) .. (445.46,74.67) -- (274.41,74.67) .. controls (271.76,74.67) and (269.6,72.51) .. (269.6,69.85) -- cycle ;
% %Rounded Rect [id:dp8359872873633009] 
% \draw   (269.13,86) .. controls (269.13,83.39) and (271.25,81.27) .. (273.86,81.27) -- (445.43,81.27) .. controls (448.05,81.27) and (450.17,83.39) .. (450.17,86) -- (450.17,100.2) .. controls (450.17,102.81) and (448.05,104.93) .. (445.43,104.93) -- (273.86,104.93) .. controls (271.25,104.93) and (269.13,102.81) .. (269.13,100.2) -- cycle ;
% %Rounded Rect [id:dp27029956856601456] 
% \draw   (268.47,137.44) .. controls (268.47,134.8) and (270.6,132.67) .. (273.24,132.67) -- (446.39,132.67) .. controls (449.03,132.67) and (451.17,134.8) .. (451.17,137.44) -- (451.17,151.76) .. controls (451.17,154.4) and (449.03,156.53) .. (446.39,156.53) -- (273.24,156.53) .. controls (270.6,156.53) and (268.47,154.4) .. (268.47,151.76) -- cycle ;
% %Rounded Rect [id:dp7324940573910047] 
% \draw   (267.8,168.83) .. controls (267.8,166.23) and (269.9,164.13) .. (272.49,164.13) -- (445.58,164.13) .. controls (448.18,164.13) and (450.28,166.23) .. (450.28,168.83) -- (450.28,182.91) .. controls (450.28,185.5) and (448.18,187.6) .. (445.58,187.6) -- (272.49,187.6) .. controls (269.9,187.6) and (267.8,185.5) .. (267.8,182.91) -- cycle ;
% %Rounded Rect [id:dp15471915563922944] 
% \draw   (268.07,200.03) .. controls (268.07,197.43) and (270.17,195.33) .. (272.76,195.33) -- (446.47,195.33) .. controls (449.07,195.33) and (451.17,197.43) .. (451.17,200.03) -- (451.17,214.11) .. controls (451.17,216.7) and (449.07,218.8) .. (446.47,218.8) -- (272.76,218.8) .. controls (270.17,218.8) and (268.07,216.7) .. (268.07,214.11) -- cycle ;
% %Straight Lines [id:da8342548459829764] 
% \draw    (58.06,115.56) -- (68.67,115.56) ;
% %Straight Lines [id:da264346558430124] 
% \draw    (70,174.22) -- (70,58.89) ;
% %Straight Lines [id:da3482901118358255] 
% \draw    (70,58.89) -- (84.72,58.89) ;
% %Straight Lines [id:da8185169417510957] 
% \draw    (70,174.22) -- (84.39,174.22) ;
% %Straight Lines [id:da5970599654535012] 
% \draw    (255,91.56) -- (255.33,30.22) ;
% %Straight Lines [id:da5677947405832151] 
% \draw    (255.33,30.22) -- (268.17,30.22) ;
% %Straight Lines [id:da08109115639970066] 
% \draw    (255,91.56) -- (268.17,91.56) ;
% %Straight Lines [id:da603888173433695] 
% \draw    (246.83,60.89) -- (268.5,60.89) ;
% %Straight Lines [id:da9668122023481845] 
% \draw    (253.67,204.89) -- (254,143.56) ;
% %Straight Lines [id:da41181555222193966] 
% \draw    (254,143.56) -- (268.17,143.56) ;
% %Straight Lines [id:da1746421482121866] 
% \draw    (253.67,204.89) -- (268.17,204.89) ;
% %Straight Lines [id:da5073022594694027] 
% \draw    (246.83,174.22) -- (268.17,174.22) ;
% %Rounded Rect [id:dp021504702174375723] 
% \draw   (461.33,24.56) .. controls (461.33,21.86) and (463.52,19.67) .. (466.23,19.67) -- (795.16,19.67) .. controls (797.86,19.67) and (800.06,21.86) .. (800.06,24.56) -- (800.06,39.24) .. controls (800.06,41.94) and (797.86,44.13) .. (795.16,44.13) -- (466.23,44.13) .. controls (463.52,44.13) and (461.33,41.94) .. (461.33,39.24) -- cycle ;
% %Rounded Rect [id:dp36019398419840787] 
% \draw   (461,57.56) .. controls (461,54.86) and (463.19,52.67) .. (465.89,52.67) -- (795.5,52.67) .. controls (798.2,52.67) and (800.39,54.86) .. (800.39,57.56) -- (800.39,72.24) .. controls (800.39,74.94) and (798.2,77.13) .. (795.5,77.13) -- (465.89,77.13) .. controls (463.19,77.13) and (461,74.94) .. (461,72.24) -- cycle ;
% %Rounded Rect [id:dp990284470711138] 
% \draw   (461.33,88.56) .. controls (461.33,85.86) and (463.52,83.67) .. (466.23,83.67) -- (794.83,83.67) .. controls (797.53,83.67) and (799.72,85.86) .. (799.72,88.56) -- (799.72,103.24) .. controls (799.72,105.94) and (797.53,108.13) .. (794.83,108.13) -- (466.23,108.13) .. controls (463.52,108.13) and (461.33,105.94) .. (461.33,103.24) -- cycle ;
% %Rounded Rect [id:dp7385353967632635] 
% \draw   (459,139.56) .. controls (459,136.86) and (461.19,134.67) .. (463.89,134.67) -- (796.16,134.67) .. controls (798.86,134.67) and (801.06,136.86) .. (801.06,139.56) -- (801.06,154.24) .. controls (801.06,156.94) and (798.86,159.13) .. (796.16,159.13) -- (463.89,159.13) .. controls (461.19,159.13) and (459,156.94) .. (459,154.24) -- cycle ;
% %Rounded Rect [id:dp09911027124281035] 
% \draw   (459.33,170.56) .. controls (459.33,167.86) and (461.52,165.67) .. (464.23,165.67) -- (794.83,165.67) .. controls (797.53,165.67) and (799.72,167.86) .. (799.72,170.56) -- (799.72,185.24) .. controls (799.72,187.94) and (797.53,190.13) .. (794.83,190.13) -- (464.23,190.13) .. controls (461.52,190.13) and (459.33,187.94) .. (459.33,185.24) -- cycle ;
% %Rounded Rect [id:dp9760277717365602] 
% \draw   (459,200.56) .. controls (459,197.86) and (461.19,195.67) .. (463.89,195.67) -- (794.83,195.67) .. controls (797.53,195.67) and (799.72,197.86) .. (799.72,200.56) -- (799.72,215.24) .. controls (799.72,217.94) and (797.53,220.13) .. (794.83,220.13) -- (463.89,220.13) .. controls (461.19,220.13) and (459,217.94) .. (459,215.24) -- cycle ;
% %Straight Lines [id:da8107566291187137] 
% \draw    (451,29.89) -- (460.94,29.89) ;
% %Straight Lines [id:da5019077435241249] 
% \draw    (451,61.56) -- (460.28,61.56) ;
% %Straight Lines [id:da15043617991990343] 
% \draw    (450.33,91.89) -- (459.61,91.89) ;
% %Straight Lines [id:da8401352624791865] 
% \draw    (451,144.89) -- (459.94,144.89) ;
% %Straight Lines [id:da41225016458038355] 
% \draw    (451.13,175.24) -- (459.61,175.24) ;
% %Straight Lines [id:da3829448090452344] 
% \draw    (451.33,205.89) -- (459.94,205.89) ;

% % Text Node
% \draw (34.83,196.23) node [anchor=north west][inner sep=0.75pt]  [rotate=-270] [align=left] {{\small Math Reasoning with LLMs}};
% % Text Node
% \draw (467.93,57.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small SelfConsistency-CoT [], Complex-CoT []}};
% % Text Node
% \draw (468.23,86.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small PAL [], PoT []}};
% % Text Node
% \draw (465.89,137.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small LLema [], MAmmoTH [], MathCoder []}};
% % Text Node
% \draw (466.89,168.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Lila []}};
% % Text Node
% \draw (465.89,198.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small ToRa []}};
% % Text Node
% \draw (90.8,164.87) node [anchor=north west][inner sep=0.75pt]   [align=left] {Knowledge Enhanced};
% % Text Node
% \draw (91.49,52.4) node [anchor=north west][inner sep=0.75pt]   [align=left] {Strategy Enhanced};
% % Text Node
% \draw (275.24,135.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {Task-specific Fine-Tuning};
% % Text Node
% \draw (275.86,84.27) node [anchor=north west][inner sep=0.75pt]   [align=left] {External Engine};
% % Text Node
% \draw (276.41,53.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Process Optimization};
% % Text Node
% \draw (276.56,22.13) node [anchor=north west][inner sep=0.75pt]   [align=left] {Prompt Engineering};
% % Text Node
% \draw (274.49,167.13) node [anchor=north west][inner sep=0.75pt]   [align=left] {Further Pre-Training};
% % Text Node
% \draw (274.76,198.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {Imitation Learning};
% % Text Node
% \draw (468.23,22.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small CoT [], ZeroShot-CoT [], Auto-CoT [], Least-to-most []}};


% \end{tikzpicture}

